IAI MovieBot: A Conversational Movie Recommender System

Conversational recommender systems support users in accomplishing recommendation-related goals via multi-turn conversations. To better model dynamically changing user preferences and provide the community with a reusable development framework, we introduce IAI MovieBot, a conversational recommender system for movies. It features a task-specific dialogue flow, a multi-modal chat interface, and an effective way to deal with dynamically changing user preferences. The system is made available open source and is operated as a channel on Telegram.

==> 00paper-02.tex <==
\section{Related work}


Relevant to our work is  ...


OpenDial~\cite{DBLP:conf/acl/LisonK16} is designed to facilitate the development of agents for single-turn Q\&A-style dialogues. However, CRS is characterized by a set of unique needs, such as making recommendations after preference elicitation, which are not well supported. Utilizing these frameworks, there exist many multi-domain, open-source CRSs such as Plato~\cite{papangelis2019collaborative} and PyDial~\cite{Ultes:2017:PMS}. These systems take the initiative to model user preference but do not track the preference evolution over conversations. Most of the available domain-specific (movie) recommender systems are closed-source commercial products, such as the Facebook messenger bot And chill.\footnote{http://www.andchill.io/} Vote GOAT~\cite{Dalton:2018:VGC} is open-sourced, but its architecture comprises commercial components like Google Dialogflow, which acquires to pay for the functionalities provided by the Dialogflow.


Our work lies at the intersection of two main research areas: recommender systems and conversational information access.
The former is the process of predicting user preferences. It aims to discover and recommend new and relevant items by content-based, collaborative filtering, or hybrid techniques. 
The latter involves the process of interpreting user utterances and disambiguating user intents, underlying users’ preferences and needs, and meeting the information needs over conversations.

\todo{Add overview of conversational recommender systems based on \citet{Jannach:2020:SCR}.}
A Conversational Recommender System (CRS) is a task-orientation system that supports its users in accomplishing recommendation-related goals through a multi-turn conversational interaction~\citep{Jannach:2020:SCR}. 
The interaction can be achieved via text-based conversation, speech or both.
%
Conversational recommender systems are proved to be more effective for more complex recommendations~\cite{kelly2013nsf} like planning a trip where multiple agents with different goals are required; or recommending a book/movie where the agent queries are mostly relevant to the current context of the system.  
The CRS are characterized as goal-driven (task-oriented) systems~\cite{Jannach:2020:SCR}, i.e., they complete a specific goal or task by making a recommendation. This characteristic differentiates the CRS from non-goal driven systems like ELIZA~\cite{weizenbaum1966eliza,DBLP:journals/cacm/Weizenbaum83}, Cleverbot~\cite{carpenter2018cleverbot} and XiaoIce~\cite{DBLP:XiaoIce} by Microsoft. Another property of CRS is a multi-turn user interaction which differentiates it from the Q\&A-style systems. Single-turn Q\&A style systems are preferred for answering simple user queries but often fail to make a recommendation after eliciting user for it's preferences. For this purpose, the multi-turn CRS maintain a dialogue state which helps with the decision-making process in the conversation.

\todo{Discuss the general frameworks and specific ones like \citep{Narducci:2018:DFB,Ultes:2017:PMS}.}
PyDial~\cite{Ultes:2017:PMS} and OpenDial~\cite{DBLP:conf/acl/LisonK16} are multi-domain frameworks for both written and spoken dialogue systems. 
Google Dialogflow is an online platform providing limited free functionalities. Although Dialogflow is widely used, it doesn't provide a room for customization of the agent and can only be used for designing and training the intents for the agent. ParlAI~\cite{DBLP:conf/emnlp/MillerFBBFLPW17} is an open-source framework by Facebook AI Research for only speech-based dialogue systems. Plato~\cite{papangelis2019collaborative} is also a multi-agent open-source framework providing a basic structure of a task-based dialogue-system for the developers.


F. Narducci et al.~\cite{Narducci:2018:DFB} proposed a domain-independent movie recommendation system\footnote{@MovieRecSysBot on Telegram} co-located with RecSys in 2018. It is a recommendation system with multiple interaction modules such as buttons and human natural language response. The general conversation comprises of asking the user to rate a few movies and based on those ratings, it can recommend a movie to the user with some major details like IMDb rating, director, actors and genres.
\todo{Discuss general tasks and used knowledge and specific task (movie rec): VoteGoat~\citep{Dalton:2018:VGC}.}
Vote GOAT~\cite{Dalton:2018:VGC} is a speech-based movie recommendation system based on Google DialogFlow. Voat GOAT recommends movies based on the user ratings and uses gamification as an incentive to receive votes for movies from the users.
\todo{This mighe be merged to intro, so either revise here or in the second paragraph in intro.}


==> 00paper-05.tex <==
\vspace*{-0.5\baselineskip}
\section{Evaluation}
For the evaluation, a feedback form\footnote{\url{https://forms.gle/q4m5fwaWMZigVsaP7}} on Google Docs is created. This form gathered basic information about the users (age, gender, and education). The users are asked to rate the system based on the quality attributes~\cite{DBLP:journals/corr/RadziwillB17} \emph{effectiveness}, \emph{efficiency} and \emph{satisfaction}. 
Moreover, the users are also inquired about what they liked and disliked most about the system. This feedback guided a better route while implementing further improvements in \emph{IAI MovieBot}~\footnote{Try this bot on \url{https://t.me/JarvisMRS\_bot} on Telegram. The command to start the conversation is \textbf{/start}.}.

\begin{figure}[ht]
\includegraphics[width=.8\linewidth]{Figures/v2_plot_likert.png}
\centering
\caption{Users' Feedback for \emph{IAI MovieBot}}
\label{fig:plot_v1}
% \vspace*{-1\baselineskip}
\end{figure}

The evaluation involved fifteen participants. Ten participants (66\%) were male, and five (33\%) were female. These participants were 25-40 years old, with an average age of 31. No participants were native English speaker, and 73\% of them had a Masters as the highest degree.
Fig \ref{fig:plot_v1} shows the ratings users provided to \emph{IAI MovieBot} based on the its \emph{effectiveness} (Q1), \emph{efficiency} (Q2-Q5) and \emph{satisfaction} (Q6-Q7). Based on the feedback and conversational data, the effectiveness of the system can be improved.





==> Tables/AgentIntentsJarvis.tex <==
\begin{table}
\caption{Overview of agent intents.  Boldfaced intents can be further split into sub-intents (listed below the dotted line).}
\scriptsize
\label{tab:AgentIntentsJarvis}
\begin{tabular}{p{1.5cm} p{6cm}}
\hline
\textbf{Intent} & \multicolumn{1}{c}{\textbf{Description}}\\
\hline
\multicolumn{2}{c}{\textbf{User Revealment~\cite{radlinski2017theoretical}/Query Formulation~\cite{trippas2018informing}}} \\ \hline
Elicit & Ask the user to describe it's information needs. \newline \say{\textit{\color{gray}Which genres do you prefer?}} or \say{\textit{\color{gray}Can you be more specific to help me narrow down the space? Give me some key words.}}\\
\hline \multicolumn{2}{c}{\textbf{System Revealment~\cite{radlinski2017theoretical}/Result Exploration~\cite{trippas2018informing}}} \\ \hline
\textbf{Reveal} & Reveal results of a count of the results in possible search space to the user \\ \hdashline
Count Results & If the list of movies matching user requirement is longer than a maximum limit. This will be followed by an Elicit intent. \newline \say{\textit{\color{gray}There are almost 1100 action movies.}}\\
Recommend & Based on information needs revealed by the user, make a recommendation.\newline \say{\textit{\color{gray}I would like to recommend a fairy tale film named Shrek.}}\\
No Results & For particular query formulated during elicitation, there can be a chance that the query results in no movies from the database. \newline \say{\textit{\color{gray}Sorry. I couldn't find any romance Korean movies.}}\\
Inform & Once the agent has revealed a result, it should be able to provide further information about the movie.\newline \say{\textit{\color{gray}The director of the recommended movie is XYZ.}} or \say{\textit{\color{gray}It was released in 1992.}}\\
\hline \multicolumn{2}{c}{\textbf{Miscellaneous Intents}} \\ \hline 
Welcome & Start the conversation by giving a short introduction \\
Acknowledge & Acknowledge the user query where required. \\
Cant Help & If the agent does not understand user query or is not able to respond properly based on it's state in the dialogue.\\
Bye & End the conversation.\\
\hline
\end{tabular}
\end{table}

==> Tables/UserIntentsJarvis.tex <==
%\newcolumntype{L}{>{\centering\arraybackslash}m{3cm}}
\begin{table}
\caption{Overview of user intents.  Boldfaced intents can be further split into sub-intents (listed below the dotted line).}
\scriptsize
\label{tab:UserIntentsJarvis}
\begin{tabular}{p{1.5cm} p{6cm}}
\hline
\textbf{Intent} & \multicolumn{1}{c}{\textbf{Description}}\\
\hline
\multicolumn{2}{l}{\textbf{User Revealment~\cite{radlinski2017theoretical} / Query Formulation~\cite{trippas2018informing} / Query Reformulation~\cite{trippas2018informing}}} \\ \hline
Reveal & Whenever the user wants to reveal any information need \newline \say{\textit{\color{gray}Do you have any sports movies?} or \textit{\color{gray}Can you also show me any recent fairy tale movie after year.}}\\
Remove \mbox{Preference} & The user wants to undo any previously revealed requirement \newline \say{\textit{\color{gray}I won't prefer any sports movies anymore.?} or \textit{\color{gray}Don't want it to be after year 2000.}}\\
\hline \multicolumn{2}{l}{\textbf{System Revealment~\cite{radlinski2017theoretical} / Result Exploration~\cite{trippas2018informing}}} \\ \hline
Inquire & Once the agent has revealed a result, the user can ask further details about the movie.\newline \say{\textit{\color{gray}Please tell me more about this one.} or \textit{\color{gray}When was this movie released?}}\\
\hline \textbf{Accept/Reject} & User decides if they like the movie recommendation or not \\ \hdashline
Accept & The user can accept the recommendation. This will determine the success of the system as finding the recommendation user likes.\newline \say{\textit{\color{gray}I like this recommendation.}}\\
Reject & Based on the agent recommendation, user may have either watched the movie or does not like it.\newline \say{\textit{\color{gray}I have already seen this one.} or \textit{\color{gray}Recommend me something else please.}}\\
Continue \mbox{Recommendation} & If the user has liked the recommendation, it can either restart, quit or continue the process and get another similar movie.\newline \say{\textit{\color{gray}I would like a similar recommendation.}}\\
\hline \multicolumn{2}{l}{\textbf{Miscellaneous Intents}} \\ \hline 
Hi & While user initiates the conversation, it starts with a formal \textit{hi/hello} then revealing preferences.\\
Acknowledge & Acknowledge the agent question where required. \\
Deny & Negate the agent question where required.\\
Bye & End the conversation by saying a bye message or exit command.\\
\hline
\end{tabular}
\end{table}
